Conditional mean embeddings as regressors - supplementary

We demonstrate an equivalence between reproducing kernel Hilbert space (RKHS) embeddings of conditional distributions and vector-valued regressors. This connection introduces a natural regularized loss function which the RKHS embeddings minimise, providing an intuitive understanding of the embeddings and a justification for their use. Furthermore, the equivalence allows the application of vector-valued regression methods and results to the problem of learning conditional distributions. Using this link we derive a sparse version of the embedding by considering alternative formulations. Further, by applying convergence results for vector-valued regression to the embedding problem we derive minimax convergence rates which are O(\log(n)/n) -- compared to current state of the art rates of O(n^{-1/4}) -- and are valid under milder and more intuitive assumptions. These minimax upper rates coincide with lower rates up to a logarithmic factor, showing that the embedding method achieves nearly optimal rates. We study our sparse embedding algorithm in a reinforcement learning task where the algorithm shows significant improvement in sparsity over an incomplete Cholesky decomposition.

==> commands.tex <==


\makeatletter

%colours
\definecolor{red}{rgb}{0.8,0.2,0.2}
\newcommand{\todo}[1]{{\color{red} {#1}}}

%environment
%\newcommand{\remark}{{\bm Remark.}}
\newcommand{\defn}{{\bf defn.\ }}

\newcommand{\I}{\mathbb{I}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\N}{\mathbb{N}}

\newcommand{\dataA}{\cD_A}
\newcommand{\dataB}{\cD_B}
\newcommand{\dataC}{\cD_C}
\newcommand{\voted}{\text{\sc voted}}
\newcommand{\spine}{{\cP_{\rm spine}}}
\newcommand{\data}{{\rm data\ }}
\newcommand{\MAP}{{\rm MAP}}
\newcommand{\interpolant}{\text{\sc interpolant}}
\newcommand{\samp}{\mathcal{S}}
\newcommand{\init}{{\rm init}}
\newcommand{\fin}{{\rm fin}}

%roman text
\newcommand{\labelled}{{\rm labelled}}
\newcommand{\unlabelled}{\rm unlabelled}
\newcommand{\normal}{\rm norm}

%metric spaces
\newcommand{\comp}{\overline}


%punctuation
\newcommand{\EQindent}{\ \ \ \ \ \ \ }
\newcommand{\ls}{``}
\newcommand{\wh}{\widehat}
\newcommand{\what}{\wh}
\newcommand{\wtilde}{\widetilde}
\newcommand{\bslash}{\backslash}

%equations
\newcommand{\bqan}{\begin{eqnarray*}}
\newcommand{\eqan}{\end{eqnarray*}}
\newcommand{\bqa}{\begin{eqnarray}}
\newcommand{\eqa}{\end{eqnarray}}
\newcommand{\bga}{\begin{align}}
\newcommand{\ena}{\end{align}}
\newcommand{\nn}{\nonumber}

%Linear Algebra and Operations
\newcommand{\diag}{{\rm diag}}
\newcommand{\row}{{\rm row}}
\newcommand{\col}{{\rm col}}
\newcommand{\lnull}{{\rm leftnull}}
\newcommand{\transpose}{\SSS \top}
\newcommand{\trans}{{\transpose}}
\newcommand{\lang}{\langle}
\newcommand{\rang}{\rangle}
\newcommand{\trace}{{\rm tr}}
\newcommand{\notbot}{\not\hspace{-1.2mm}\bot}

\newcommand{\spec}{{\rm spec}}
\newcommand{\Image}{{\rm im}}
\newcommand{\Ext}{{\rm Ext}}


%punctuation
\newcommand{\upto}{,...}

\newcommand{\sgn}{{\rm sgn}}
\newcommand{\DDt}{\frac{\rm d}{{\rm d}t}}

%sets
\newcommand{\cZtest}{\cZ_{{\rm test}}}
\newcommand{\cZtrain}{\cZ_{{\rm train}}}
\newcommand{\cHt}{\widetilde \cH}
\newcommand{\Kt}{\widetilde K}

%minimisers
\newcommand{\empmin}{h^*}
\newcommand{\subempmin}{{\overline h}^*}
\newcommand{\realmin}{h^*}
\newcommand{\subrealmin}{{\overline h}^*}

%networks
\newcommand{\source}{{\rm source}}
\newcommand{\sink}{{\rm sink}}
\newcommand{\netw}{\mathcal{N}}


%Bold and curlies and romans and hats

\newcommand{\rd}{{\rm d}}
\newcommand{\dd}{{\rm d}}

\newcommand{\barn}{{\bar n}}

\newcommand{\hh}{\what h}
\newcommand{\hn}{{\what n}}
\newcommand{\bhh}{\what {\bm h}}
\newcommand{\bhg}{\what {\bm g}}
\newcommand{\chX}{\what \cX}
\newcommand{\bhk}{{\what \bk}}
\newcommand{\bhK}{{\what \bK}}
\newcommand{\bhQ}{{\what \bQ}}

\newcommand{\bLambda}{\bm \Lambda}
\newcommand{\bPhi}{\bm \Phi}
\newcommand{\bPsi}{\bm \Psi}
\newcommand{\bP}{\bm P}
\newcommand{\bL}{\bm L}
\newcommand{\bD}{\bm D}
\newcommand{\bA}{\bm A}
\newcommand{\bff}{\bm f}
\newcommand{\ba}{\bm a}
\newcommand{\bg}{\bm g}
\newcommand{\bK}{\bm K}
\newcommand{\bI}{\bm I}
\newcommand{\bd}{\bm d}
\newcommand{\bv}{\bm v}
\newcommand{\bR}{\bm R}
\newcommand{\bQ}{\bm Q}
\newcommand{\bk}{\bm k}
\newcommand{\bx}{{\bm x}}
\newcommand{\bh}{{\bm h}}
\newcommand{\bX}{{\bm X}}
\newcommand{\by}{\bm y}
\newcommand{\bz}{\bm z}
\newcommand{\bU}{\bm U}
\newcommand{\bu}{\bm u}
\newcommand{\bT}{\bm T}
\newcommand{\bM}{\bm M}
\newcommand{\bw}{\bm w}
\newcommand{\bS}{\bm S}
\newcommand{\bW}{\bm W}
\newcommand{\bZ}{\bm Z}
\newcommand{\be}{\bm e}
\newcommand{\bb}{\bm b}
\newcommand{\bc}{\bm c}
\newcommand{\bp}{\bm p}
\newcommand{\bs}{\bm s}
\newcommand{\bJ}{\bm J}
\newcommand{\bF}{\bm F}
\newcommand{\bG}{\bm G}
\newcommand{\bH}{\bm H}
\newcommand{\bE}{\bm E}
\newcommand{\bC}{\bm C}
\newcommand{\bcL}{\bm {\mathcal L}}
\newcommand{\bxi}{\bm \xi}
\newcommand{\bmu}{\bm \mu}
\newcommand{\bDelta}{{\bm \Delta}}
\newcommand{\btheta}{{\bm \theta}}
\newcommand{\balpha}{{\bm \alpha}}
\newcommand{\bbeta}{{\bm \beta}}
\newcommand{\bone}{\bm 1}
\newcommand{\blambda}{{\bm \lambda}}
\newcommand{\bsigma}{{\bm \sigma}}
\newcommand{\bSigma}{{\bm \Sigma}}
\newcommand{\bXi}{{\bm \Xi}}
\newcommand{\bgamma}{{\bm \gamma}}
\newcommand{\bepsilon}{\bm \epsilon}
\newcommand{\bnabla}{\bm \nabla}
\newcommand{\bzeta}{\bm \zeta}
\newcommand{\bpi}{\bm \pi}
\newcommand{\cM}{{\mathcal M}}
\newcommand{\cN}{{\mathcal N}}
\newcommand{\cA}{{\mathcal A}}
\newcommand{\cV}{{\mathcal V}}
\newcommand{\cR}{{\mathcal R}}
\newcommand{\cH}{{\mathcal H}}
\newcommand{\cG}{{\mathcal G}}
\newcommand{\cC}{{\mathcal C}}
\newcommand{\cX}{{\mathcal X}}
\newcommand{\cQ}{{\mathcal Q}}
\newcommand{\cY}{{\mathcal Y}}
\newcommand{\cO}{{\mathcal O}}
\newcommand{\cI}{{\mathcal I}}
\newcommand{\cL}{{\mathcal L}}
\newcommand{\cT}{{\mathcal T}}
\newcommand{\cP}{{\mathcal P}}
\newcommand{\cK}{{\mathcal K}}
\newcommand{\cS}{{\mathcal S}}
\newcommand{\cE}{{\mathcal E}}
\newcommand{\cW}{{\mathcal W}}
\newcommand{\cF}{{\mathcal F}}
\newcommand{\cU}{{\mathcal{U}}}
\newcommand{\cB}{{\mathcal B}}
\newcommand{\cD}{{\mathcal D}}
\newcommand{\cZ}{{\mathcal Z}}
\newcommand{\cXY}{\cX\times\cY}


%special vectors
\newcommand{\point}[2]{{\left(\ap_{#1}({#2})\right)}}
\newcommand{\bpoint}[2]{{\ap_{#1}({#2})}}

\newcommand{\ap}{\bP}

\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\argsup}{\operatornamewithlimits{argsup}}
%complexity
\newcommand{\Cut}{{\rm cut}}
\newcommand{\sparsity}{s}
\newcommand{\cut}{\Phi}
\newcommand{\cond}{\gamma}
\newcommand{\Cond}{\Gamma}
\newcommand{\ratio}{r}

%Graph Structure
\newcommand{\length}{\ell}
\newcommand{\dist}{d}
\newcommand{\diam}{D}
\newcommand{\wD}{\Delta}
\newcommand{\res}{r}
\newcommand{\RES}{R}
\newcommand{\pres}{\res_p}
\newcommand{\presG}{\res_{\cG,p}}
\newcommand{\pRES}{\RES_p}
\newcommand{\cover}{\cC}

\newcommand{\pred}{{\hat{y}}}
\newcommand{\predt}{ {\hat{y}_t} }
\newcommand{\Tr}{{\rm Tr}}
\newcommand{\reals}{\R}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\lnorm}{||\by||^2_L}
\newcommand{\nchoosec}{\left( ^{n}_{c} \right)}
\newcommand{\prob}{{\rm Prob}}
\newcommand{\rank}{{\rm rank}}
\newcommand{\spann}{{\rm span}}
\newcommand{\degree}{{\rm degree}}

\newcommand{\thresh}{{\rm thresh}}
\newcommand{\pow}{P}


%learning
\newcommand{\trainv}{\{(v_{i_1},y_1),(v_{i_2},y_2),...(v_{i_T},y_T)\}}
\newcommand{\trainx}{\{(x_{i_1},y_1),(x_{i_2},y_2),...(x_{i_T},y_T)\}}

%%% Mark defines
\newcommand{\Proj}{{\rm proj}}
\newcommand{\proj}[2]{{{\rm proj}_{\cmap,p}({#2;#1})}}
\newcommand{\projF}[2]{{{\rm proj}_{F}({#2;#1})}}
\newcommand{\norm}[1]{{\|{#1}\|}}
\newcommand{\SSS}{\scriptscriptstyle}
\newcommand{\bzero}{\mathbf 0}
\newcommand{\wt}{ \mbox{\boldmath$w$}_t }
\newcommand{\wts}{ \mbox{\boldmath$w$}_{t+1} }


\newcommand{\prj}{\rm proj}

\newcommand{\cmap}{\bm \Psi}
\newcommand{\cmapc}{\Psi}
%norms
\newcommand{\smoothness}[1]{S_{\cG} {#1}}
\newcommand{\pnorm}[1]{{\|{#1}\|_p}}
\newcommand{\pnormq}[1]{{\|{#1}\|^2_p}}
\newcommand{\cpnorm}[1]{{\|{#1}\|_{\cmap,p}}}
\newcommand{\cpnormSqr}[1]{{\|{#1}\|^2_{\cmap,p}}}
\newcommand{\cpnormg}[1]{{\|{#1}\|_{\cmap_{\cG},p}}}
\newcommand{\cpnormGraph}[1]{{\|{#1}\|_{\cG,p}}}
\newcommand{\cqnormGraph}[1]{{\|{#1}\|_{\cG,q}}}
\newcommand{\ctnormGrapht}[1]{{\|{#1}\|_{\cG,2}^2}}
\newcommand{\cpnormGraphp}[1]{{\|{#1}\|^p_{\cG,p}}}
\newcommand{\cpnormGraphSqr}[1]{{\|{#1}\|^2_{\cG,p}}}
\newcommand{\cpnormGraphDashp}[1]{{\|{#1}\|^p_{\cG',p}}}
\newcommand{\cpnormq}[1]{{\|{#1}\|^2_{\cmap,p}}}
%conjugate norms
\newcommand{\cqnorm}[1]{{\|{#1}\|_{\cmap,q}}}
\newcommand{\normConj}[1]{\norm{#1}^*}
\newcommand{\cqnormSqr}[1]{{\|{#1}\|^2_{\cmap,q}}}
\newcommand{\cqnormGraphSqr}[1]{{\|{#1}\|^2_{\cG,q}}}
\newcommand{\cqnormg}[1]{{\|{#1}\|_{\cmap_{\cG},q}}}
\newcommand{\cpnormgConj}[1]{{\|{#1}\|^*_{\cmap_{\cG}}}}
\newcommand{\cpnormGraphConj}[1]{{\|{#1}\|^*_{\cG,p}}}
\newcommand{\cpnormGraphConjSqr}[1]{{\|{#1}\|^{*^{2}}_{\cG,p}}}
%\newcommand{\cpnormGraphConjSqr}[1]{({\|{#1}\|^{*}_{\cG,p}})^2}
\newcommand{\cpnormConj}[1]{{\|{#1}\|^*_{\cmap,p}}}
\newcommand{\cpnormConjSqr}[1]{{\|{#1}\|^{*^2}_{\cmap,p}}}

\newcommand{\dvg}{{\rm div}}


\newcommand{\into}{\rightarrow}
\newcommand{\GG}{{\mathbf G}}

\newcommand{\bset}{\mathcal{S}}
\newcommand{\pf}{E}

%risk and loss
\newcommand{\lossz}{{\ell}_{0-1}}
\newcommand{\loss}{{\ell}}
\newcommand{\risk}{{\rm risk}}
\newcommand{\riskl}{{\risk^\loss}}
\newcommand{\rempl}{\widehat {\risk}_\loss}
\newcommand{\rempli}{\widehat {\risk}^{(i)}_\loss}
\newcommand{\riskt}{\risk_{\cT}}
\newcommand{\remp}{{\widehat \risk}}
\newcommand{\trs}{{\rm trs}}
\newcommand{\ind}{{\rm ind}}
\newcommand{\rempls}{\widehat{\rm risk}\vspace{-0.1cm}^{ \loss}_{\hspace{-0.04cm}\cS}\vspace{0.1cm}}
\newcommand{\remps}{\widehat{\rm risk}_{\cS}}
\newcommand{\remplsi}{\widehat{\rm risk}\vspace{-0.1cm}^{ \loss}_{\hspace{-0.04cm}\cS^{(i)}}\vspace{0.1cm}}
\newcommand{\risklt}{{\risk^\loss_\cT}}
\newcommand{\risklst}{{\risk^\loss_{\cS\cup\cT}}}

%smoothness and regularization
\newcommand{\semp}{\widehat U_{\cS}}
\newcommand{\sempT}{\widehat U_{\cT}}
\newcommand{\sempi}{\widehat U_{\cS^{(i)}}}
\newcommand{\sempdash}{\widehat U_{\cS'}}
\newcommand{\smooth}{U}
\newcommand{\reg}{{\rm reg}}


\newcommand{\sempInst}{\twiddle U _\cI}

%probability
\newcommand{\Expect}{\E}
\newcommand{\Prob}{\P}
\newcommand{\Bin}{ {\rm Bin}}
\newcommand{\kl}{{\rm kl}}
\newcommand{\cov}{{\rm cov}}
\newcommand{\var}{{\rm var}}
\newcommand{\lkl}{{\rm kl}}
\newcommand{\bKL}{{\rm KL}}
\newcommand{\Boltz}{{\rm boltz}}
\newcommand{\Opt}{{\rm opt}}
\newcommand{\Cat}{{\rm opt}}
\newcommand{\post}{Q}
\newcommand{\Joint}{\widehat Q}

%random variables
\newcommand{\rad}{\sigma}
\newcommand{\brad}{\bsigma}

%function class complexity
\newcommand{\VC}{\VCdim}
\newcommand{\VCdim}{{\rm VC}}
\newcommand{\mRad}{\cR_m}
\newcommand{\EmpRad}{\widehat \cR}
\newcommand{\mRadTrs}{\cR^{\rm trs}_m}
\newcommand{\mRadInd}{\cR^{\rm ind}_m}
\newcommand{\RadTrs}{\cR^{\rm trs}}
\newcommand{\Rad}{\cR}

\newcommand{\mGaussn}{\cG_m}
\newcommand{\EmpGauss}{\widehat\cG}

%Symbols
\newcommand{\twiddle}{\widetilde}

\newcommand{\regQ}{F_Q}
\newcommand{\regP}{F_P}

%footnotes

\newcommand{\footnoteremember}[2]{\footnote{#2}
  \newcounter{#1}
  \setcounter{#1}{\value{footnote}}
} 

\newcommand{\footnoterecall}[1]{\footnotemark[\value{#1}]} 

